Decoupled Prioritized Resampling for Offline RL

Offline reinforcement learning (RL) is challenged by the distributional shift problem. To address this problem, existing works mainly focus on designing sophisticated policy constraints between the learned policy and the behavior policy. However, these constraints are applied equally to well-performing and inferior actions through uniform sampling, which might negatively affect the learned policy. To alleviate this issue, we propose Offline Prioritized Experience Replay (OPER), featuring a class of priority functions designed to prioritize highly-rewarding transitions, making them more frequently visited during training. Through theoretical analysis, we show that this class of priority functions induce an improved behavior policy, and when constrained to this improved policy, a policy-constrained offline RL algorithm is likely to yield a better solution. We develop two practical strategies to obtain priority weights by estimating advantages based on a fitted value network (OPER-A) or utilizing trajectory returns (OPER-R) for quick computation. OPER is a plug-and-play component for offline RL algorithms. As case studies, we evaluate OPER on five different algorithms, including BC, TD3+BC, Onestep RL, CQL, and IQL. Extensive experiments demonstrate that both OPER-A and OPER-R significantly improve the performance for all baseline methods. Codes and priority weights are availiable at https://github.com/sail-sg/OPER.

==> rebuttal_materials/compare_AW.tex <==



\centering
\captionof{table}{Compare AW and OPER-R with IQL on Antmaze.}
\label{tab:mix}
\begin{tabular}{c l cc  }
\toprule
&           & AW & OPER-R  \\
\midrule
\multirow{6}{*}{\rotatebox[origin=c]{90}{antmaze}}
&umaze          &        \textbf{90.7}        & 87.8           \\
&umaze-diverse  &      \textbf{75.3}        & 66.0           \\
&medium-play    &      61.3    & \textbf{72.0}          \\
&medium-diverse &       22   & \textbf{74.2}  \\
&large-play     &      23.3       & \textbf{49.6}  \\
&large-diverse  &      9.3   & \textbf{43.0}           \\
\rowcolor[HTML]{EFEFEF}
&antmaze total  &     281.9    & \textbf{392.6} \\
\bottomrule
\end{tabular}
\vspace{7mm}


% \begin{table}[htbp]
% \vspace{-1mm}

%  \caption{}
%   \vspace{2mm}

% \begin{subtable}[b]{0.55\textwidth}
% \scriptsize
% \centering
% \caption{OPER-A on 50\% Transition Dataset with 10 seeds.}
% \label{tab:random}
% \begin{tabular}{ccccc}
% \toprule
% \multirow{2}{*}{50\% Dataset} & \multicolumn{2}{c}{TD3+BC}     & \multicolumn{2}{c}{IQL}  \\
% \cmidrule(lr){2-3}\cmidrule(lr){4-5}
%                          & vanilla       & OPER-A         & vanilla & OPER-A         \\
% \midrule

% halfcheetah-m        & 48.5          & \textbf{49.9}  & 44.1    & \textbf{47.3}  \\
% hopper-m             & 60.4          & \textbf{72.9}  & 57.0    & \textbf{68.8}  \\
% walker2d-m           & 66.0          & \textbf{82.5}  & 67.7    & \textbf{81.7}  \\
% halfcheetah-mr       & 43.2          & \textbf{45.2}  & 35.5    & \textbf{39.2}  \\
% hopper-mr            & 76.4          & 74.9           & 78.5    & \textbf{91.2}  \\
% walker2d-mr          & 53.3          & \textbf{89.6}  & 55.6    & \textbf{75.2}  \\
% halfcheetah-me       & \textbf{89.1} & 77.7           & 90.8    & 89.9           \\
% hopper-me            & 100.0         & \textbf{108.4} & 106.9   & 108.9          \\
% walker2d-me          & 110.3         & \textbf{111.6} & 109.4   & \textbf{112.2} \\
% \rowcolor[HTML]{EFEFEF}
% total                & 647.2         & \textbf{712.7} & 645.5   & \textbf{714.4} \\
% \rowcolor[HTML]{EFEFEF}
% SD (total)           & 25.2          & 13.1           & 23.9    & 14.7  \\
% \bottomrule    
% \end{tabular}
% \end{subtable}
% \hfill
% \begin{subtable}[b]{0.43\textwidth}
% \centering
% \caption{Compare AW and OPER-R with IQL on Antmaze.}
% \label{tab:mix}

% \begin{tabular}{c l cc  }
% \toprule
% &           & AW & OPER-R  \\
% \midrule
% \multirow{6}{*}{\rotatebox[origin=c]{90}{antmaze}}
% &umaze          &        \textbf{90.7}        & 87.8           \\
% &umaze-diverse  &      \textbf{75.3}        & 66.0           \\
% &medium-play    &      61.3    & \textbf{72.0}          \\
% &medium-diverse &       22   & \textbf{74.2}  \\
% &large-play     &      23.3       & \textbf{49.6}  \\
% &large-diverse  &      9.3   & \textbf{43.0}           \\
% \rowcolor[HTML]{EFEFEF}
% &antmaze total  &     281.9    & \textbf{392.6} \\
% \bottomrule
% \end{tabular}
% \end{subtable}
  

% \end{table}


==> rebuttal_materials/finegrain_and_aw.tex <==

\begin{figure}[ht]
\vspace{-10mm}
  \begin{minipage}{0.49\textwidth}
\scriptsize
\centering
\captionof{figure}{The toy example to illustrate the capability of OPER-A to concatenate trajectories, thereby creating enhanced behaviors.}
\includegraphics[width=0.98\textwidth]{rebuttal_materials/concat_traj.pdf}
\label{tab:random}

\end{minipage}%
\hfill
\begin{minipage}{0.49\textwidth}
\centering


\captionof{table}{Compare OPER against percentage sampling with hyperparameter search (10 seeds).}
\begin{tabular}{c|cc}
\toprule
 & TD3+BC               & IQL                  \\
\midrule
1\%                  & 241.2±12.6           & 226.8±19.4           \\
10\%                 & 602.1±23.9           & 654.3±7.9            \\
25\%                 & 675.9±18.4           & 681.3±9.1            \\
50\%                 & 692.6±19.3           & 697.2±10.2           \\
75\%                 & 679.5±11.1           & 681.2±14.1           \\
vanilla (100\%)      & 669.7± 17.1          & 682.1± 22.3          \\
\midrule
OPER-A               & \textbf{734.1± 10.4} & \textbf{727.8± 11.2} \\
OPER-R               & \textbf{707.3± 7.9}  & \textbf{726.7± 8.9} \\
\bottomrule
\end{tabular}

\end{minipage}
\end{figure}


==> table/decouple.tex <==

\begin{table}[t]\centering
% \small
% \scriptsize
\caption{Averaged normalized scores over the final 10 evaluations and 5 seeds on D4RL tasks except for Antmaze. we report the final evaluation and 5 seeds for Antmaze. Following IQL, we use "v2" environments for mujoco tasks and "v0" for other tasks.
}\label{tab:decouple}
\begin{tabular}{c l c c c c}
\toprule
&                                & IQL   & \nameno & \ournameno &  \\
% halfcheetah-medium                  &    47.6  & 47.6  \\               
% hopper-medium                        &   64.3   &  66 \\ 
% walker2d-medium                      &    79.9  &  78.6 \\ 
% halfcheetah-medium-replay            &    43.4  &  44.3 \\ 
% hopper-medium-replay                 &    89.1  &  101 \\ 
% walker2d-medium-replay               &    69.6  &  79.5 \\ 
% halfcheetah-medium-expert            &    83.5  &  92.6 \\ 
% hopper-medium-expert                 &    96.1  &  106.1 \\ 
% walker2d-medium-expert               &    109.2  & 110.5  \\ 
\midrule
&mujoco total                     &  682.7  & \textbf{726.2} & \textbf{722.1} \\ 
\midrule
\multirow{6}{*}{\rotatebox[origin=c]{90}{antmaze}}
&umaze                           &  88  & 89.2 &  89.6 \\
&umaze-diverse                   &  64  & \textbf{79.8} &  72.3 \\
&medium-play                     &   71.5 & \textbf{78.4} &  71.8 \\
&medium-diverse                 &  57.5  & 68.4 &  \textbf{77.6} \\
&large-play                     &   42.3 & 14.6 &  \textbf{49.2} \\
&large-diverse                  &  44  & 37.6 &  \textbf{48.2} \\
\midrule
&antmaze total                  &   367.3 & 368 &  \textbf{408.7} \\
\midrule
&kitchen total                  &  169.1  & \textbf{182.1} &  \textbf{179.5} \\
&adroit total                   &  125.2 & \textbf{161.7} &  \textbf{156.3} \\
\midrule
&total                          &  1344.3  & 1438.0 &  \textbf{1466.6} \\
\midrule
&     runtime                 &   28min   &  29min  &  40min \\
\bottomrule
\end{tabular}
\end{table}

==> table/full_result.tex <==

\begin{table}[h]\centering
% \small
% \scriptsize
\caption{Full Results of ? and ? on D4RL. 
}\label{tab:full}
\begin{booktabs}{
  colspec = {lccccc},
%   cell{1,2,3}{4} = {c=2}{c}, % multicolumn (column number=2, center alignment)
}
\toprule
                                & IQL   & ? & \SetCell[c=2]{c} {{{?}}} & & ?-A \\
\cmidrule[lr]{4-5} \cmidrule[lr]{6}
                                &       &          & stage1 & stage2 & stage2 \\

\midrule                                
halfcheetah-medium                   &    47.6  & 47.6   & 47.5 & 47.6 & 47.7  \\               
hopper-medium                        &    64.3   &  66   & 65.5 & 65.1 & 66.1 \\ 
walker2d-medium                      &    79.9  &  78.6  & 74.5 & 81.9$\uparrow$ & 81\\ 
halfcheetah-medium-replay            &    43.4  &  44.3  & 43.9 & 43.4 & 43.5 \\ 
hopper-medium-replay                 &    89.1  &  101   & 92.8 & 100.1$\uparrow$ & 94.8\\ 
walker2d-medium-replay               &    69.6  &  79.5  & 72.9 &  77$\uparrow$ & 76.8\\ 
halfcheetah-medium-expert            &    83.5  &  92.6  & 87.9 &  91.8$\uparrow$ & 91.2 \\ 
hopper-medium-expert                 &    96.1  &  106.1 & 89.3 & 104.7$\uparrow$ & 104.5\\ 
walker2d-medium-expert               &    109.2  & 110.5 & 110.1 &  722.1 & 110.1 \\ 
\midrule
mujoco total                     &  682.7  & \textbf{726.2} & 684.4 & \textbf{722.1$\uparrow$} & 715.5 \\ 
\midrule
antmaze total                  &   367.3 & 368 & 376.2 & \textbf{408.7}$\uparrow$ & 390.6 \\
\midrule           
kitchen-complete-v0              & 66.3 &  62.7  & 67.4	 &  64 & 63.2\\
kitchen-partial-v0              & 53.3 & 69.5 &	47.6	& 66$\uparrow$ & 67.3\\
kitchen-mixed-v0                & 49.5	& 49.9 & 50.9	& 49.5 & 47.7\\ \midrule   
kitchen-v0 total                &  169.1  & \textbf{182.1} & 165.9 &  \textbf{179.5$\uparrow$} & \textbf{178.2}\\ \midrule
pen-human-v0                     & 74.8 & 83 & 76 & 88$\uparrow$ & 83  \\
hammer-human-v0                   & 1.7	& 1.8 &	1.5	& 2.1 & 1.7 \\
door-human-v0                     & 4.3 &	4.4	& 6.1 & 7.1  & 5.8 \\
relocate-human-v0                 & 0.1 &	0.1 &	0.1 &	0.1  & 0.1 \\
pen-cloned-v0                     & 40.9 & 66.6 & 37.8 &	53$\uparrow$   & 46.4  \\
hammer-cloned-v0                  & 1.8 &	1.1 &	1.6 &	1.8  & 5.3    \\
door-cloned-v0                    & 1.8 &	4.9 &	2.4 &	4.4   & 3.9   \\
relocate-cloned-v0                &  -0.2 &	-0.2 &	-0.2 &	-0.2 & -0.2\\ \midrule
adroit-v0 total                 &  125.2 & \textbf{161.7} & 125.3 &  \textbf{156.3$\uparrow$} & 146 \\
\midrule
total                          &  1344.3  & 1438.0 & 1351.8 & \textbf{1466.6} & 1430\\
\bottomrule
\end{booktabs}
\end{table}

==> table/nstep=5.tex <==
\begin{table}[h]
\small
\scriptsize
% \vspace{-15pt}
 \centering
\caption{The effect of advantage estimators. Experiments are conducted on IQL (\shortalgo). We use multi-step bootstrap (N=1 or 5) to fit value function and compute advantage.}
\label{tab:nstep=5}
\scalebox{0.88}{
\begin{tabular}{c|ccc}
\toprule
   & vanilla & N=1 & N=5 \\
\midrule
kitchen-complete-v0 & 65.9  & 74.3   &     64.2    \\
kitchen-partial-v0  & 51.4  & \textcolor{red}{38.8} &    66.5     \\
kitchen-mixed-v0    & 50.3  & \textcolor{red}{26.0} &  52.1 \\ 
\midrule  
kitchen total    & 167.6 & 139.1 & 182.8 \\
\midrule
\midrule
pen-human-v0   & 73.1  & \textcolor{red}{60.8} &    72.9          \\
pen-cloned-v0  & 42.1  & 53.6 &   61.2        \\
\bottomrule
\end{tabular}
}
\vspace{-15pt}
\end{table}

==> table/p_base.tex <==

\begin{table}[h]\centering
% \small
% \scriptsize
\caption{Effect of hyperparamter $p_{base}$.
}\label{tab:p_base}
\begin{booktabs}{
  colspec = {lcccc},
}
\toprule
$p_{base}$                            & 0   & 0.2 & 0.5  & 1.0 & $\infty$ (IQL) \\
\midrule                                
halfcheetah-medium                   &   47.6   &   - & 47.4 &   - & 47.6 \\               
hopper-medium                        &   66   &  -  & 64.1 &  -   & 64.3 \\   
walker2d-medium                      &   78.6   &  -  & 78.9 &   - & 79.9 \\   
halfcheetah-medium-replay            &   44.3   &  -  & 44.3 &   -  & 43.4 \\   
hopper-medium-replay                 &   101   &  -  & 99.2 &  -   & 89.1 \\   
walker2d-medium-replay               &   79.5   &  -  & 61.3 &  -  & 69.6 \\   
halfcheetah-medium-expert            &    92.6  & -   & 90.6 &  -   & 83.5 \\   
hopper-medium-expert                 &    106.1  &  -  & 84.9 &   - & 96.1 \\    
walker2d-medium-expert               &    110.5  &  -  & 110.1 &   - & 109.2\\ 
\midrule
mujoco total                     &   726.2   &  -  & 680.8 &   - & 682.7 \\   
\midrule
antmaze-umaze                         & 86.8 &	89.2 &	85.6 &	91.4 &	88  \\   
antmaze-umaze-diverse                &   37	& 79.8 &	65.8 &	60.4 &	64 \\   
antmaze-medium-play                  &   37.6 &	78.4 &	72.8 &	72.2 &	71.5 \\   
antmaze-medium-diverse               &  32.8 &	68.4 &	64 &	74.2 &	57.5  \\  
antmaze-large-play                   &  23.4 &	14.6 &	20.6 &	24.4 &	42.3 \\   
antmaze-large-diverse               &  24.4 &	37.6 &	42.4 &	44.4 &	44  \\   
\midrule
antmaze total                       &  242 &	368 &	351.2 &	367 &	367.3 \\
\bottomrule
\end{booktabs}
\end{table}

==> table/priority-indicator.tex <==

% \begin{table}[h]\centering
% % \small
% % \scriptsize
% \caption{Full Results of rebalance and decouple on D4RL. 
% }\label{tab:cql}
% \begin{tabular}{lccccc}
% \toprule
%                                 & CQL   & CQL[rebalance] & CQL[10\%] & CQL[50\%] & reward-rebalance\\
% \midrule                                
% halfcheetah-medium                   & 48.1	& 48.2 &	47 &	48.3 &	48.2  \\               
% hopper-medium                       & 71.8	& 69.4 &	65.5 &	69.9 &	68.2 \\ 
% walker2d-medium                     &  83.3 &	83.5 &	76.5 &	80.4 &	83 \\ 
% halfcheetah-medium-replay           &  45.2	& 46.3 &	41.8 &	45.3 &	46.4\\ 
% hopper-medium-replay                &  95.3	& 98.6 &	96.8 &	97.6 &	97.7\\ 
% walker2d-medium-replay              &  82.3 &	86.7 &	67.9 &	78.1 &	83.9\\ 
% halfcheetah-medium-expert          &  66.2 &	81.6 &	73.3 &	89 &	74.2 \\ 
% hopper-medium-expert             &    76.9 &	95 &	106.6 &	108.4 &	87\\ 
% walker2d-medium-expert             &   110 &	110	 & 109.3 &	108.9 &	109.4 \\ 
% \midrule
% mujoco total                    & 679.1	 & 719.3 &	684.7 &	725.9 &	698\\
% \bottomrule
% \end{tabular}
% \end{table}


\begin{table}[ht]\centering
% \small
% \scriptsize
\caption{The effect of different prioritization strategies. }
\label{tab:priority-indicator}
\resizebox{0.55\textwidth}{!}{
\begin{booktabs}{
%   colspec = {l|cccc|cccc},
%   cell{1}{2,6} = {c=4}{c}, % multicolumn (column number=2, center alignment)
colspec = {l|cccc},cell{1}{2} = {c=4}{c}}
\toprule
        & CQL   &  &  & \\
\cmidrule[lr]{2-5}
& vanilla   & \shortalgoo & 10\%return  &  \shortname-reward \\
\midrule  
halfcheetah-medium                   & 48.1	& 48.2 &	47.0 &	48.2  \\               
hopper-medium                       & 71.8	& 69.4 &	65.5 &	68.2 \\ 
walker2d-medium                     &  83.3 &	83.5 &	76.5 &		83.0 \\ 
halfcheetah-medium-replay           &  45.2	& 46.3 &	41.8 &	46.4\\ 
hopper-medium-replay                &  95.3	& 98.6 &	96.8 &		97.7\\ 
walker2d-medium-replay              &  82.3 &	86.7 &	67.9 &		83.9\\ 
halfcheetah-medium-expert          &  66.2 &	81.6 &	73.3 &	74.2 \\ 
hopper-medium-expert             &    76.9 &	95.0 &	106.6 &	87.0\\ 
walker2d-medium-expert             &   110.0 &	110.0	 & 109.3 &	109.4 \\ 
\midrule
mujoco total                    & 679.1	 & 719.3 &	684.7  &	698.0\\
\bottomrule
\end{booktabs}}
\end{table}

==> table/two_algos.tex <==
\begin{table}
\begin{center}
\vspace{-2mm}
% \scriptsize\
\small
\caption{A summary for two  algorithms.}
\label{table:two-algos}
\begin{tabular}{ccc}
\toprule
 & \shortalgo & \shortalgoo \\
\midrule
Prerequisite  & None & full trajectory \\
\midrule
Extra Runtime  & fit value function  &  $< 3 $ seconds \\
\midrule
% Effect  & \multicolumn{2}{c}{boost performance by a large margin} \\
% \midrule
\multirow{2}{*}{\centering Features}  & \multicolumn{2}{c}{decoupled resampling;} \\
    & \multicolumn{2}{c}{weights can be reused}      \\
\bottomrule
\end{tabular}
\vspace{-2mm}
\end{center}
\end{table}
